Beneath Surface Similarity: Large Language Models Make Reasonable Scientific Analogies after Structure Abduction

The vital role of analogical reasoning in human cognition allows us to grasp novel concepts by linking them with familiar ones through shared relational structures. Despite the attention previous research has given to word analogies, this work suggests that Large Language Models (LLMs) often overlook the structures that underpin these analogies, raising questions about the efficacy of word analogies as a measure of analogical reasoning skills akin to human cognition. In response to this, our paper introduces a task of analogical structure abduction, grounded in cognitive psychology, designed to abduce structures that form an analogy between two systems. In support of this task, we establish a benchmark called SCAR, containing 400 scientific analogies from 13 distinct fields, tailored for evaluating analogical reasoning with structure abduction. The empirical evidence underlines the continued challenges faced by LLMs, including ChatGPT and GPT-4, in mastering this task, signifying the need for future exploration to enhance their abilities.

==> table/050ScienceQA.tex <==
% Table generated by Excel2LaTeX from sheet 'scienceQA'


% Table generated by Excel2LaTeX from sheet 'scienceQA'
\begin{table*}[t]
  \centering
    \small
    \begin{tabular}{lcccccc}
    \toprule
       \multicolumn{1}{c}{\multirow{2}[0]{*}{\textbf{Model}}}    & \multicolumn{2}{c}{\textbf{NAT}} & \multicolumn{2}{c}{\textbf{SOC}} & \multicolumn{2}{c}{\textbf{LAN}}\\
       \cmidrule{2-7}
         &\textbf{Acc. }$\uparrow$  & ($\Delta$ $\uparrow$)&\textbf{Acc. }$\uparrow$  & ($\Delta$ $\uparrow$) &\textbf{Acc. }$\uparrow$  & ($\Delta$ $\uparrow$) \\
    \midrule
    \rowcolor[gray]{0.95} \multicolumn{7}{c}{\textit{Zero-Shot In-context Learning}}\\
    InstructGPT$_\texttt{002}$~\cite{lu2022learn}   & 75.04  &   -    & \textbf{66.28}  &   -    & \textbf{77.27}  & - \\
    \ \ w/  \texttt{CoT} & 77.80  & (2.76)  & 65.61  & (-0.67)  & 76.82  & (-0.45)  \\
    \ \ w/  \texttt{Analogy} & 78.24  & (3.20)  & 67.74  & (1.46)  & 76.36  & (-0.91)  \\
    \ \ w/  \texttt{Analogy with example} & \textbf{78.42}  & (3.38)  & 66.06  & (-0.22)  & 76.82  & (-0.45) \\
    \midrule
    InstructGPT$_\texttt{003}$~\cite{ouyang2022training}   & 75.36  &   -    & \textbf{67.06}  &   -    & \textbf{77.45}  & - \\
    \ \ w/  \texttt{CoT} & 77.04  & (1.68)  & 67.06  & (0.00)  & 76.82  & (-0.63) \\
    \ \ w/  \texttt{Analogy} & 78.15  & (2.79)  & 67.84  & (0.78)  & 76.18  & (-1.27) \\
    \ \ w/  \texttt{Analogy with example} & \textbf{78.20}  & (2.84)  & 66.61  & (-0.45)  & 76.73  & (-0.72)  \\
    \midrule
    ChatGPT~\cite{openai2022chatgpt} & 66.70  &     -  & 67.39  &    -   & \textbf{78.20}  & - \\
    \ \ w/  \texttt{CoT} & 72.87  & (6.17)  & \textbf{69.42}  & (2.03)  & 74.95  & (-3.25)   \\
    \ \ w/  \texttt{Analogy} & \textbf{73.53}  & (6.83)  & 67.62  & (0.23)  & 73.89  & (-4.31)  \\
    \ \ w/  \texttt{Analogy with example} & 73.31  & (6.61)  & 69.08  & (1.69)  & 74.63  & (-3.57) \\
    \midrule
    \rowcolor[gray]{0.95} \multicolumn{7}{c}{\textit{Supervised Learning}} \\
    %UnifiedQA~\cite{khashabi-etal-2020-unifiedqa} & 68.16 & - & 69.18& - & 74.91& - \\ 
    Multimodal-CoT~\cite{zhang2023multimodal} & 87.52& - & 77.17 & - & 85.82 & -   \\
    LLaMA-Adapter~\cite{zhang2023llama} & 84.37 & - & 88.30 & - & 84.36 & -   \\
    \midrule
    Human~\cite{lu2022learn} & 90.23 & - & 84.97 & - & 87.48 & -    \\
    \bottomrule
    \end{tabular}%
    \caption{Accuracy (\textbf{Acc.}) of different models on the ScienceQA dataset across natural science (NAT), social science (SOC), and language science (LAN) domains.
    We report the accuracy gap ($\Delta$) between vanilla LLMs and LLMs with hints.
    The best results of LLMs with different hints are \textbf{bolded}.}
  \label{tab:scienceqa}%
\end{table*}%



\begin{comment}
    \begin{table*}[t]
  \centering
    \small
    \begin{tabular}{lccccccc}
    \toprule
       \multicolumn{1}{c}{\multirow{2}[0]{*}{\textbf{Model}}}    & \multicolumn{2}{c}{\textbf{NAT}} & \multicolumn{2}{c}{\textbf{SOC}} & \multicolumn{2}{c}{\textbf{LAN}} & \multicolumn{1}{c}{\multirow{2}[0]{*}{\textbf{AVG}}}\\
       \cmidrule{2-7}
         &\textbf{Acc. }$\uparrow$  & ($\Delta$ $\uparrow$)&\textbf{Acc. }$\uparrow$  & ($\Delta$ $\uparrow$) &\textbf{Acc. }$\uparrow$  & ($\Delta$ $\uparrow$) \\
    \midrule
    \rowcolor[gray]{0.95} \multicolumn{8}{c}{\textit{Zero-Shot In-context Learning}}\\
    InstructGPT$_\texttt{002}$~\cite{lu2022learn}   & 75.04  &   -    & \textbf{66.28}  &   -    & \textbf{77.27}  & - & 72.83\\
    \ \ w/  \texttt{CoT} & 77.80  & (2.76)  & 65.61  & (-0.67)  & 76.82  & (-0.45)  & 73.41\\
    \ \ w/  \texttt{Analogy} & 78.24  & (3.20)  & 67.74  & (1.46)  & 76.36  & (-0.91)  & \textbf{74.11}\\
    \ \ w/  \texttt{Analogy with example} & \textbf{78.42}  & (3.38)  & 66.06  & (-0.22)  & 76.82  & (-0.45)  & 73.77\\
    \midrule
    InstructGPT$_\texttt{003}$~\cite{ouyang2022training}   & 75.36  &   -    & \textbf{67.06}  &   -    & \textbf{77.45}  & - & 73.29\\
    \ \ w/  \texttt{CoT} & 77.04  & (1.68)  & 67.06  & (0.00)  & 76.82  & (-0.63)  & 73.64\\
    \ \ w/  \texttt{Analogy} & 78.15  & (2.79)  & 67.84  & (0.78)  & 76.18  & (-1.27)  & \textbf{74.06}\\
    \ \ w/  \texttt{Analogy with example} & \textbf{78.20}  & (2.84)  & 66.61  & (-0.45)  & 76.73  & (-0.72)  & {73.85}\\
    \midrule
    ChatGPT~\cite{openai2022chatgpt} & 66.70  &     -  & 67.39  &    -   & \textbf{78.20}  & - & 70.76\\
    \ \ w/  \texttt{CoT} & 72.87  & (6.17)  & \textbf{69.42}  & (2.03)  & 74.95  & (-3.25)  &\textbf{72.41} \\
    \ \ w/  \texttt{Analogy} & \textbf{73.53}  & (6.83)  & 67.62  & (0.23)  & 73.89  & (-4.31)  & 71.68 \\
    \ \ w/  \texttt{Analogy with example} & 73.31  & (6.61)  & 69.08  & (1.69)  & 74.63  & (-3.57)  & 72.34\\
    \midrule
    \rowcolor[gray]{0.95} \multicolumn{8}{c}{\textit{Supervised Learning}} \\
    %UnifiedQA~\cite{khashabi-etal-2020-unifiedqa} & 68.16 & - & 69.18& - & 74.91& - & 70.75  \\ 
    Multimodal-CoT~\cite{zhang2023multimodal} & 87.52& - & 77.17 & - & 85.82 & - & 83.50   \\
    LLaMA-Adapter~\cite{zhang2023llama} & 84.37 & - & 88.30 & - & 84.36 & - & 85.68   \\
    \midrule
    Human~\cite{lu2022learn} & 90.23 & - & 84.97 & - & 87.48 & - & 87.56   \\
    \bottomrule
    \end{tabular}%
    \caption{Accuracy (\textbf{Acc.}) of different models on the ScienceQA dataset across natural science (NAT), social science (SOC), and language science (LAN) domains.
    We report the accuracy gap ($\Delta$) between vanilla LLMs and LLMs with hints.
    The best results of LLMs with different hints are \textbf{bolded}.}
  \label{tab:scienceqa}%
\end{table*}%

\end{comment}

==> table/080template_scienceqa.tex <==
\begin{table*}[t]
  \centering
  \small
    \begin{tabular}{l}
    \toprule
    \makecell[l]{
    \color{gray}{/* \textit{Task prompt} */}\\
    Please answer the following question.\\
    \color{gray}{/* \textit{Question} */}\\
    Question: Does this passage describe the weather or the climate?\\ Where Darnel lives, winter is the rainiest season of the year.\\
    Options: (A) weather (B) climate \\
    \color{gray}{/* \textit{Answer} */} \\
    Answer: \color[rgb]{0,0.39,0}\textit{(A) weather.} \\
    \midrule
    \color{gray}{/* \textit{Hint: Step~\cite{kojima2022large}} */} \\
    Hint: you can think step by step. \\
    \color{gray}{/* \textit{Answer} */} \\
    Answer: \color[rgb]{0,0.39,0}\textit{(A) weather. The passage describes a specific season (winter) and a specific aspect of that season (raininess), which}\\ \color[rgb]{0,0.39,0}\textit{is a characteristic of the weather rather than the long-term patterns of climate.}\\
    \midrule
    \color{gray}{/* \textit{Hint: Work out~\cite{zhou2023large}} */} \\
    Hint: Let's work this out in a step by step way to be sure we have the right answer. \\
    \color{gray}{/* \textit{Answer} */} \\
    Answer: \color[rgb]{0,0.39,0}\textit{This passage describes the climate.}\\
    \midrule
    \color{gray}{/* \textit{Hint: Plan~\cite{wang2023plan}} */} \\
    Hint: Let's first understand the problem and devise a plan to solve the problem. Then, let's carry out the plan and solve the\\ problem step by step. \\
    \color{gray}{/* \textit{Answer} */} \\
    Answer: \\
    \color[rgb]{0,0.39,0}\textit{Plan:}\\
    \color[rgb]{0,0.39,0}\textit{Darnel lives in a place that has seasonal changes; this means that the weather changes from time to time. However, the} \\
    \color[rgb]{0,0.39,0}\textit{passage says that winter is the rainiest season of the year. What does this imply? This implies that the passage is not talking} \\
    \color[rgb]{0,0.39,0}\textit{about weather changes, but rather the typical pattern of weather in this place. This is what we call a climate pattern. There is} \\
    \color[rgb]{0,0.39,0}\textit{still a possibility that it can be weather, but let's take this as an assumption.}\\
    \color[rgb]{0,0.39,0}\textit{Carry out the Plan:}\\
    \color[rgb]{0,0.39,0}\textit{Let's go to answer choices.}\\
    \color[rgb]{0,0.39,0}\textit{(A) weather: This choice goes against our assumption. It states that the passage is talking about the currently occurring} \\
    \color[rgb]{0,0.39,0}\textit{atmosphere of Darnel's place. However, the passage says that winter is the rainiest season of the year, indicating a long-term} \\
    \color[rgb]{0,0.39,0}\textit{pattern of weather rather than the weather that occurs during the time of writing the passage. Therefore, this choice is}\\
    \color[rgb]{0,0.39,0}\textit{incorrect. (B) climate: This choice supports our assumption made in the plan. It states that the passage is talking about the} \\
    \color[rgb]{0,0.39,0}\textit{long-term pattern of weather in Darnel's place. This is the correct choice.}\\
    \color[rgb]{0,0.39,0}\textit{Therefore, the answer is (B) climate.}\\
    \midrule
    \color{gray}{/* \textit{Hint: Analogy} */} \\
    Hint: you can answer the question with the help of useful analogies. \\
    \color{gray}{/* \textit{Answer} */} \\
    Answer: \color[rgb]{0,0.39,0}\textit{(B) climate. The passage describes a pattern of weather (rainy season in winter) that is typical for the area, which is}\\ \color[rgb]{0,0.39,0}\textit{characteristic of climate. An analogy could be that the weather on a particular day is like a snapshot, while climate is like}\\ \color[rgb]{0,0.39,0}\textit{a photo album of weather patterns over time.}\\
    \midrule
    \color{gray}{/* \textit{Hint: Analogy with Example} */} \\
    Hint: you can answer the question with the help of useful analogies. For example, taking the analogy of the camera structure is \\helpful for people to understand the properties of the eye. \\
    \color{gray}{/* \textit{Answer} */}\\
    Answer: \color[rgb]{0,0.39,0}\textit{(B) climate. Just as the weather on a given day is like a snapshot and the climate is like a photo album of weather} \\\color[rgb]{0,0.39,0}\textit{patterns over time, The passage describes the weather over time, hence the climate.}} \\
    \bottomrule
    \end{tabular}
  \caption{Instruction template and hints for LLMs in science question answering. Generated texts by LLMs (ChatGPT in this table) are {\color[rgb]{0,0.39,0}\textit{highlighted}}.
  }
  \label{tab:scienceqa_template}
\end{table*}


==> table/150ScienceQA_cot.tex <==
% Table generated by Excel2LaTeX from sheet 'scienceQA'


% Table generated by Excel2LaTeX from sheet 'scienceQA'
\begin{table*}[t]
  \centering
    \small
    \begin{tabular}{lcccccc}
    \toprule
       \multicolumn{1}{c}{\multirow{2}[0]{*}{\textbf{Model}}}    & \multicolumn{2}{c}{\textbf{NAT}} & \multicolumn{2}{c}{\textbf{SOC}} & \multicolumn{2}{c}{\textbf{LAN}} \\
       \cmidrule{2-7}
         &\textbf{Acc. }$\uparrow$  & ($\Delta$ $\uparrow$)&\textbf{Acc. }$\uparrow$  & ($\Delta$ $\uparrow$) &\textbf{Acc. }$\uparrow$  & ($\Delta$ $\uparrow$) \\
    \midrule
    InstructGPT$_\texttt{002}$   & 75.04  &   -    & 66.28  &   -    & 77.27  & - \\
    \ \ w/  Step & 77.80  & (2.76)  & 65.61  & (-0.67)  & 76.82  & (-0.45)  \\
    \ \ w/  Work Out & 74.16  & (-0.88)  & 64.45  & (-1.83)  & 76.64  & (-0.63)    \\
    \ \ w/  Plan & 73.85  & (-1.19)  & 61.30  & (-4.98)  & 77.18  & (-0.09)    \\
    \midrule
    InstructGPT$_\texttt{003}$   & 75.36  &   -    & 67.06  &   -    & 77.45  & - \\
    \ \ w/  Step & 77.04  & (1.68)  & 67.06  & (0.00)  & 76.82  & (-0.63)  \\
    \ \ w/  Work Out & 74.16  & (-1.20)  & 64.23  & (-2.83)  & 76.09  & (-1.36)    \\
    \ \ w/  Plan & 73.36  & (-2.00)  & 60.85  & (-6.21)  & 78.36  & (0.91)   \\
    \midrule
    ChatGPT & 66.70  &     -  & 67.39  &    -   & 78.20  & -\\
    \ \ w/  Step & 72.87  & (6.17)  & 69.42  & (2.03)  & 74.95  & (-3.25)   \\
    \ \ w/  Work Out &   64.43  & (-2.27)  & 57.93  & (-9.46)  & 66.45  & (-11.75)   \\
    \ \ w/  Plan &  72.34  & (5.64)  & 60.74  & (-6.65)  & 75.52  & (-2.68)   \\
    \bottomrule
    \end{tabular}%
    \caption{Accuracy (\textbf{Acc.}) of LLMs with different zero-shot reasoning prompts on the ScienceQA dataset across natural science (NAT), social science (SOC), and language science (LAN) domains.}
  \label{tab:scienceqa_cot}%
\end{table*}%

\begin{comment}
    \begin{table*}[t]
  \centering
    \small
    \begin{tabular}{lccccccc}
    \toprule
       \multicolumn{1}{c}{\multirow{2}[0]{*}{\textbf{Model}}}    & \multicolumn{2}{c}{\textbf{NAT}} & \multicolumn{2}{c}{\textbf{SOC}} & \multicolumn{2}{c}{\textbf{LAN}} & \multicolumn{1}{c}{\multirow{2}[0]{*}{\textbf{AVG}}}\\
       \cmidrule{2-7}
         &\textbf{Acc. }$\uparrow$  & ($\Delta$ $\uparrow$)&\textbf{Acc. }$\uparrow$  & ($\Delta$ $\uparrow$) &\textbf{Acc. }$\uparrow$  & ($\Delta$ $\uparrow$) \\
    \midrule
    InstructGPT$_\texttt{002}$   & 75.04  &   -    & 66.28  &   -    & 77.27  & - & 72.83\\
    \ \ w/  Step & 77.80  & (2.76)  & 65.61  & (-0.67)  & 76.82  & (-0.45)  & 73.41\\
    \ \ w/  Work Out & 74.16  & (-0.88)  & 64.45  & (-1.83)  & 76.64  & (-0.63)  & 71.75  \\
    \ \ w/  Plan & 73.85  & (-1.19)  & 61.30  & (-4.98)  & 77.18  & (-0.09)  & 70.78  \\
    \midrule
    InstructGPT$_\texttt{003}$   & 75.36  &   -    & 67.06  &   -    & 77.45  & - & 73.29\\
    \ \ w/  Step & 77.04  & (1.68)  & 67.06  & (0.00)  & 76.82  & (-0.63)  & 73.64\\
    \ \ w/  Work Out & 74.16  & (-1.20)  & 64.23  & (-2.83)  & 76.09  & (-1.36)  & 71.49  \\
    \ \ w/  Plan & 73.36  & (-2.00)  & 60.85  & (-6.21)  & 78.36  & (0.91)  & 70.86  \\
    \midrule
    ChatGPT & 66.70  &     -  & 67.39  &    -   & 78.20  & - & 70.76\\
    \ \ w/  Step & 72.87  & (6.17)  & 69.42  & (2.03)  & 74.95  & (-3.25)  &72.41 \\
    \ \ w/  Work Out &   64.43  & (-2.27)  & 57.93  & (-9.46)  & 66.45  & (-11.75)  & 62.94  \\
    \ \ w/  Plan &  72.34  & (5.64)  & 60.74  & (-6.65)  & 75.52  & (-2.68)  & 69.53  \\
    \bottomrule
    \end{tabular}%
    \caption{Accuracy (\textbf{Acc.}) of LLMs with different zero-shot reasoning prompts on the ScienceQA dataset across natural science (NAT), social science (SOC), and language science (LAN) domains.}
  \label{tab:scienceqa_cot}%
\end{table*}%
\end{comment}





